Path integrals for classical-quantum dynamics

Consistent dynamics which couples classical and quantum degrees of freedom exists. This dynamics is linear in the hybrid state, completely positive and trace preserving. Starting from completely positive classical-quantum master equations, we derive a general path integral representation for such dynamics in terms of a classical-quantum action, which includes the necessary and sufficient conditions for complete positivity and trace preservation. The path integral we study is a generalization of the Feynman path integral for quantum systems, and the stochastic path integral used to study classical stochastic processes, allowing for interaction between the classical and quantum systems. When the classical-quantum Hamiltonian is at most quadratic in the momenta we are able to derive a configuration space path integral, providing a map between master equations and covariant classical-quantum path integrals.

==> quicksummary.tex <==
\section{Quick Summary}

The path integral for classical dynamics with diffusion in $p$, e.g. corresponding to Brownian motion such as
\begin{align}
    \frac{\partial \rho}{\partial t}=\{H,\rho\}+\frac{\partial^2 D_2 \rho}{\partial p^2}
\end{align}
is given by
\begin{align}
\rho(p, t)=& \lim _{N \rightarrow \infty} \int_{N \text { times }} \int \prod_{i=0}^{N-1}\left\{\left[4 \pi D_{2}\left(p_{i}, t_{i}\right) \tau\right]^{-1 / 2} \mathrm{~d} x_{i}\right\} 
%\\& 
\times \exp \left(-\sum_{i=0}^{N-1} \frac{\left[p_{i+1}-p_{i}+\frac{\partial H}{\partial q}\left(p_{i}, t_{i}\right) \tau\right]^{2}}{4 D_2\left(p_{i}, t_{i}\right) \tau}\right) \rho\left(p_{0}, t_{0}\right)
\end{align}
where $\rho\left(p_{0}, t_{0}\right)$ is the initial probability density of $p$, and $\rho(p, t)$ the one at $t$.
It is clearly positive. The term in the exponent is called the Onsager-Machlup function, and taking the limit $N\rightarrow\infty$, is
\begin{align}
-\int_{t_{0}}^{t} \frac{\left[\dot{p}\left(t^{\prime}\right)+\frac{\partial H}{\partial q}\left(p\left(t^{\prime}\right), t^{\prime}\right)\right]^{2}}{4 D_2\left(p\left(t^{\prime}\right), t^{\prime}\right)} \mathrm{d} t^{\prime}
\end{align}
where we have written
$
p_{i+1}-p_{i}=\dot{p}\left(t_{i}\right) \tau
$. We will be calling this the ''action'' $\mathcal{I}$.
 The book of Riskin on the Fokker-Planck equation has an easily accessible introduction to it on p 73 and this Wikipedia entry \url{https://en.wikipedia.org/wiki/Fokker-Planck_equation}is not bad.
 
 Note that as $D_2$ goes to $0$, the momentum follows it's deterministic path, but otherwise has a broadening variance around it.
An example of a Lorentz invariant stochastic path integral for a classical scalar field is given by the "action" 
[INSERT]



Next, going to the purely quantum case, recall that we can write the action for an example of a Lorentz invariant Lindblad Equation by doubling the fields (call them $\xql$ and $\xqr$) to get the action
\begin{equation}
\begin{split}
    &  \mathcal{I}( \xql,  \xqr,t_i,t_f) =    \int_{t_i}^{t_f} dt\bigg[   iL_+  - iL_- - \frac{D_0}{2}\int dx \left(\xql(x)-\xqr(x)\right)^2
   % -\frac{1}{2}(\frac{ \delta  \Delta W_I}{ \delta q_{\alpha}}) D_0^{\alpha \beta} ( \frac{\delta \Delta W_I}{ \delta q_{\beta}})
    \bigg].
    \end{split}
\end{equation} 
Since we are interested in Lindblad operators of the form $\frac{\partial V_I}{\partial q_\alpha}$ and their field-theoretic version, we can write the Lindbladian action as
\begin{equation}
\begin{split}
    &  \mathcal{I}( \xql,  \xqr,t_i,t_f) =    \int_{t_i}^{t_f} dt\bigg[   iL_+  - iL_- 
    -\frac{1}{2}(\frac{ \delta  \Delta W_I}{ \delta q_{\alpha}}) D_0^{\alpha \beta} ( \frac{\delta \Delta W_I}{ \delta q_{\beta}})
    \bigg].
    \end{split}
\end{equation} 
where $\Delta W_I:=V_-V_-$ is the different of the left and right potentials.

Now we want to find the path integral for classical-quantum dynamics whose master equation is Equation \eqref{eq: withLindblad} 
\begin{equation}%\label{eq: withLindblad}
\begin{split}
    \frac{\partial \cqstate(\q,\p)}{\partial t} & = \{H_c, \cqstate \} -i[H_q,\cqstate]  + \frac{\partial^2 }{\partial \p_i \partial  \p_j }( D_{2,ij}(
    \q_i) \cqstate)+  \frac{1}{2} \left( \{ V_{I}(\q_i,\xq), \cqstate \}  - \{\cqstate, V_I(\q_i, \xq) \} \right)  \\
    & + D_0^{\alpha \beta} (\q_i)\left( \frac{\partial V_I}{\partial q_{\alpha}} \cqstate\frac{\partial V_I^{\dag}}{\partial q_{\beta}} - \frac{1}{2} \{\frac{\partial V_I^{\dag}}{\partial q_{\beta}} \frac{\partial V_I}{\partial q_{\alpha}} , \cqstate \} \right)
\end{split}
\end{equation}
The first two terms are the usual deterministic classical and quantum ones, the third term is the classical diffusion term, the fourth term gives the back reaction of the interaction potential and the final term is a Lindbladian. The matrices $D_2$ and $D_0$ (or kernels in the field theory case) have to satisfy certain conditions for the dynamics to be Completely Positive Trace Preserving (CPTP).


Its
path integral
will combine the stochastic classical path integral and the doubled quantum one, and it's action is initially given as Equation \ref{eq: continuousActionHamiltonian}
\begin{equation}%\label{eq: continuousActionHamiltonian}
\begin{split}
    &  \mathcal{I}( \xql,  \xqr,   \pql,  \pqr,  \q, \p ,t_i,t_f) =    \int_{t_i}^{t_f} dt\bigg[ + i\dot{\xqr}\pqr - iH^{\rind}  - i\dot{\xql}\pql + iH^{\lind}  \\
    & -\frac{1}{2}( \frac{ \partial V_I^{\lind}}{\partial q_{\alpha}} - \frac{\partial V_I^{\rind}}{\partial q_{\alpha}}) D_0^{\alpha \beta} (\q,t)( \frac{ \partial V_I^{\lind}}{\partial q_{\beta}} - \frac{\partial V_I^{\rind}}{\partial q_{\beta}}) \\
    &  - \frac{1}{2} \log(\operatorname{det} D_2(\q,t)) - \frac{1}{2} \left(\dot{\p}_i + \frac{\partial H_c}{\partial \q_i} + \frac{1}{2 } \frac{\partial V_{I}^{\lind}}{\partial \q_i} + \frac{1}{2 } \frac{\partial V_{I}^{\rind}}{\partial \q_i}\right)D_{2, ij}^{-1}(\q,t)\left(\dot{\p}_j + \frac{\partial H_c}{\partial \q_j} + \frac{1}{2 } \frac{\partial V_{I}^{\lind}}{\partial \q_j} + \frac{1}{2 } \frac{\partial V_{I}^{\rind}}{\partial \q_j}\right)  
    \bigg].
\end{split}
\end{equation} 
and after performing some integrals, becomes the configuration space action of Equation \ref{eq: continuousActionPositionSpace2}.

Next, let's move to gravity. The most promising example from  \cite{Oppenheim:2018igd} has the master equation
    \begin{align}
\frac{\partial\cqstate(g,\pi,t)}{\partial t} = &
\{H[N,\vec{N}],\cqstate\}
-i  \left[\qhamint[N,\vec{N}],\cqstate  \right]
+\frac{1}{2} \left(\{\qhamint[N,\vec{N}](x),\cqstate\}-\{\cqstate,\qhamint[N,\vec{N}]\}\right)
\nonumber\\
&
+\frac{1}{2} \int 
dxdy 
D_{0,\mu\nu\sigma\tau}(g,N;x,x') \left[\L^{\mu\nu}(N;x),\left[\cqstate,\L^{\sigma\tau}(N;x)\right]\right]
+\frac{1}{2} \int 
dx dx' 
 \{N(x) J_\alpha(g;x),\{D_2\ab (N;x,y)J_\beta(g;x'),\cqstate\}\}
\nonumber\\
\label{eq:dynamicsPQG-continuous}
\end{align}
with $\qhamint$ the matter Hamiltonian, $H[N,\vec{N}]$ the ADM Hamiltonian, the $J$ being scalar densities, e.g. $\sqrt{g}$ or $\sqrt{g}^{(3)}R$ (or even the superHamiltonian, although I think this would be problematic). I've computed the constraint structure taking $D_2$ to only depend on $N$ implicitly, and the Linblad operators to be
\begin{align}
\L(x)=g_{ij}\frac{\delta \qham(x)}{\delta g_{ij}}-\frac{1}{2}\qham(x)
\end{align} 
thus leaving $D_{0,\mu\nu\sigma\tau}(g,N;x,x')$ to just be some $D_2(x,x')N(x)$. It would be great if we could take them to be delta functions, but I prefer to leave them general, since all one is sacrificing is cluster decomposition rather, and the dynamics themselves are local. I've played with various other positions of the lapse(s), but I think this one can be justified. The action, is then given by Equation \eqref{eq: continuousActionFinal}. Just to be explicit, 
%\begin{equation}\label{eq: continuousActionFinalIntro}
%\begin{split}
 %   &  \mathcal{I}( \xql,  \xqr,   \pql,  \pqr,  \z,t_i,t_f) =    \int_{t_i}^{t_f} dt dx \bigg[ - \frac{1}{2} \log(\operatorname{det} \lambda^+)\delta(x)  -\frac{1}{2} D_{1}^{diff \dag}(x) \cdot D_2^{-1}(x) \cdot D_{1}^{diff}(x) \\
  %  & i\dot{\xqr}\pqr(x) - i\mathcal{H}^+(x)  - i\dot{\xql}\pql(x) + i\mathcal{H}^- + D^{\alpha %\beta}_0(x)  L_{\alpha}^{\rind}(x) L_{\beta}^{* \lind}(x)- \frac{1}{2} D^{\alpha \beta}_0(x) \left( L^{*\lind}_{\beta}(x)L_{\alpha}^{\lind}(x) + L^{*\rind}_{\beta}(x)L_{\alpha}^{\rind}(x) \right) \bigg].
 %   \end{split}
%\end{equation} 
for a single, Hermitian, Lindblad operator, as above, and taking the $D_i$ to be delta functions, this reduces to 
\begin{equation}\label{eq: continuousActionFinalIntro2}
\begin{split}
    &  \mathcal{I}( \xql,  \xqr,   \pql,  \pqr,  \z,t_i,t_f) =    \int_{t_i}^{t_f} dt N dx \bigg[ - \frac{1}{2} \log(\operatorname{det} D_2)(x) -\frac{1}{2} D_{1}^{diff \dag}(x) \cdot D_2^{-1}(x) \cdot D_{1}^{diff}(x) \\
    & i\dot{\xqr}\pqr(x) - i\mathcal{H}^+(x)  - i\dot{\xql}\pql(x) + i\mathcal{H}^-  -\frac{1}{2}D_0(x)(L^+- L^-)^2 \bigg].
    \end{split}
\end{equation} 
Here, $D_2$. $D_1^{diff}$ is a vector which acts to suppress paths differening from their left/right averaged Hamiltonian equations of motion 
\begin{equation}
    D_{1,1}^{diff}(z) = \{z_i, H_c \} + \frac{1}{2}\{z_i,H_m^-\} + \frac{1}{2}\{z_i,H_m^+\} - \frac{dz_i}{dt} 
\end{equation} and the det of $D_2$ will have some power of $N$ which looks worrying, and either requires gauge fixing, or a tier of constraints (which might be okay since these are constraints on the density matrix).

We also weren't sure how to integrate out the momentum degrees of freedom, perhaps you have some insight here? Alternatively, one could just try to write down a diffeomorphism action, as in Equations \eqref{eq:KGaction} and \eqref{eq:PQG-action}, but it's unclear how to see that the dynamics is CP. It sounded like you thought this might be relatively easy. My suspicion is that it won't be CP, because one has some mixed signature, in the same way that $\partial_\mu(\xql-\xqr) \partial^\mu(\xql-\xqr)$. However, I have to admit, I'm not so bothered by breaking space-time diff invariance, as long as it satisfies some weaker projected symmetry e.g.  in terms of the algebra of the dynamical generators of time translation as we discussed.



==> relmeasscrap.tex <==
\subsection{Lorentz invariant measurement dynamics}
As we saw in section \ref{sec: derivationContinuous}, when the classical degrees of freedom are taken to be measurement signals, the CQ path integral describes a path integral over all possible measurement signals, as well as quantum trajectories. In the field theoretic case, the measurement signals are instead described by fields $z(x)$, as are the quantum operators being measured. We shall show that we can write down Lorentz invariant measurement dynamics for measurement of any operator which depends on the quantum field. The measurement dynamics we find has a Lorentz invariant action, includes collapse, and is to be understood in the full field theoretic case, and compliments other discussions on relativistic measurement \cite{RovMarolf2002, PhilippsLorentzInv,2002Reisenberger}.

In the field theoretic case, we would like to arrive at some form of measurement dynamics. In general, the \textit{outcomes} of measurements - even continuous measurements - are discontinuous in time. In continuous measurement and feedback, this is generally why it is preferred to study the evolution and feedback using measurement signals $dz_t = \alpha_t dt$ which are better behaved \cite{Wiseman_2001, 2006Jacob}. We could try to consider the field theoretic version of Equation \eqref{eq: state} for a Hermitian operator $Z(z(x))$ which can depend on the classical measurement signal $z(x)$ at time $t$, as can its strength $k(z)$. We could then formally write down the field theoretic version of Equation \eqref{eq: continuousMeasuAction}. However, it appears that an immediate problem arises if we wish the action to be Lorentz invariant since the dynamics in Equation \eqref{eq: measurement outcome1} involves a single time derivative of the classical variable $z(x)$. This problem arises because in the measurement dynamics of Equation's \eqref{eq: state}, \eqref{eq: measurement outcome1} the equation of motion for the measurement signal \eqref{eq: measurement outcome1} is first order in time. One option to obtain a Lorentz \textit{covariant} path integral is to contract this with a preferred frame field $n^{\mu} \partial_{\mu} z(x)$, but this will not be Lorentz invariant unless $n^{\mu}$ is itself dynamical.\footnote{Note, one cannot leave the indices free $\partial_{\mu}z(x)$ and contract the back-reaction term with the Minkowski metric, since it is not positive definite and the dynamics will not be CP.} 

However, we have already seen that Equation  \eqref{eq: LorentzInvariantAction} can give rise to Lorentz invariant dynamics, and its important to see how Equation \eqref{eq: LorentzInvariantAction} avoids these problems: the dynamics for the classical variable is second order in time. In particular, replacing $\q \to z$ and $\phi \to Z(\phi)$ and $\lambda \to 1$ the path integral in Equation \eqref{eq: LorentzInvariantAction} is equivalent to the following set of stochastic differential equations 
\begin{align}\label{eq: statefield}
& \frac{\partial|\psi(t)\rangle}{\partial t}= -iH |\psi(t)\rangle - \left\{-k(z_t)(Z(z_t)-\langle Z(z_t) \rangle )^{2} +\sqrt{2 k(z_t)}(Z(z_t)-\langle Z(z_t)\rangle) J(t,x) \right\}|\psi(t)\rangle,\\
&
\label{eq: measurement outcome1field}
\partial_{\mu} \partial^{\mu}z(t,x) =\langle Z(z_t)\rangle +\frac{J(t,x)}{\sqrt{8 k(z_t)}},
\end{align}
when the decoherence diffusion trade-off is satisfied. Here $J(x)$ is a white noise process satisfying $\mathbb{E}[J(t,x)]=0$, $\mathbb{E}[J(t,x) J(t',x')] = \delta(t-t')\delta(x-x')$, and $D_0(z) = 2k(z), D_2(z) = \frac{1}{8k(z)}$. To see the equivalence between Equation's \eqref{eq: statefield}, \eqref{eq: measurement outcome1field} and the action \eqref{eq: LorentzInvariantAction}, one use the white noise statistics to find the dynamics for the CQ state in Equation \eqref{eq: CQstateDefinition}, which takes the form of Equation \eqref{eq: fieldConfigurationSpaceME} \cite{UCLHealing}. Hence, despite being motivated by the CQ master Equation in \eqref{eq: fieldConfigurationSpaceME}, the path integral \ref{eq: LorentzInvariantAction} has an equivalent interpretation in terms of a continuous measurement procedure, where one consider a continuous measurement and feedback via a non-standard measurement signal $z(x)$ via Equation \eqref{eq: measurement outcome1field}. We emphasize that these equations are actually more general than measurement of a standard Hermitian observable $Z$, since they also allow for the case where there is Markovian feedback which depends on the measurement signal $z(x)$. If there is no feedback, then the variables, and Hermitian operator, appearing in Equation \eqref{eq: state} will not be $z$ dependent, in which case it corresponds to a pure measurement procedure. We should also emphasize that when no-measurement is being performed, i.e, $k(z_t)=0$, we have pure unitary evolution on the quantum state.

In analogy with the standard continuous measurement equations, Equation \eqref{eq: state} also gives rise to dynamics for the collapse of the wave-vector and conditioned on a particular measurement value $z(x)$, one can uniquely update the quantum state by inverting $J(t,x)$ in terms of $z(t,x)$. The measurement signal, which can be used for Markovian feedback and control on the quantum state is sourced by the measurement outcome $\alpha(t,x)$ via Equation \eqref{eq: measurement outcome1field}. We could of course try to construct a path integral for the measurement outcome 
\begin{equation}
    \alpha(t,x)  = \langle Z(z_t)\rangle +\frac{J(t,x)}{\sqrt{8 k(z_t)}},
\end{equation}directly, but this is technically more difficult, because it is widely discontinuous. 

Nonetheless, given the measurement record $z(x)$ one can find the measurement outcome by applying the Lorentz invariant operator $\partial_{\mu} \partial^{\mu}$ to the measurement signal $\partial_{\mu} \partial^{\mu} z(t,x) = \alpha(t,x)$. As such, describing measurement outcomes in terms of $z(t,x)$ or $\alpha(t,x)$ should be  physically equivalent descriptions of the measurement procedure. In some sense, working with the measurement signal $z(t,x)$ is simply a type of regularization procedure to ensure which ensures that the resulting path integral is continuous and we can make analytical progress. 

Equation's \eqref{eq: statefield}, \eqref{eq: measurement outcome1field} therefore appear to define Lorentz invariant measurement dynamics. Specifically, the classical-quantum transition amplitude, which describes probability distribution over classical measurement signals as well as their associated quantum trajectories is determined by a Lorentz invariant action, which we can out explicitly as
\begin{equation}\label{eq: LorentzInvariantActionMeasurement}
\begin{split}
     \mathcal{I}( Z^{\pm}, z ,t_i,t_f) & =    \int_{t_i}^{t_f} dt d \vec{x} \bigg[   iL_{Q}^+(x)  - iL_{Q}^-(x)     -4 k(z)( \partial_{\mu}\partial^{\mu}z)^2 + 4k(z )( \partial_{\mu}\partial^{\mu} z)( Z^+(z,\phi)+ Z^{-}(z,\phi)) \\
     & - 2k(z)( (Z^{+})^2+ (Z^{-})^2)
     - \frac{1}{2}\log( D_2[z])
    \bigg].
    \end{split}
\end{equation}
Note because the decoherence diffusion trade-off is saturated, this path integral further factorizes into $\pm$ branches, but we see that the evolution of each branch is not unitary. In particular, defining 
\begin{equation}\label{eq: simpleLorentzinvmeasaction}
    \mathcal{I}_{CQ}[z,\phi]= \int_{t_i}^{t_f} dt d\vec{x} \big[iL_{Q}(x) +4k(z) ( \partial_{\mu}\partial^{\mu} z)Z-2k(z) Z^2  \big]
\end{equation}
and 
\begin{equation}
    \mathcal{I}_{C}[z] =  \int_{t_i}^{t_f} dt d \vec{x} \big[ 4 k(z)( \partial_{\mu}\partial^{\mu}z)^2 + \frac{1}{2}\log( D_2[z]) \big]
\end{equation}
the path integral can be written 
in the form of Equation \eqref{eq: positiveCQfields}.

Equivalently, the dynamics for the measurement procedure is described via Equation's \eqref{eq: statefield}, \eqref{eq: measurement outcome1field}, and the measurement outcome can be obtained by applying the Lorentz invariant operator to the measurement signal $\partial_{\mu}\partial^{\mu} z(x)$. Since the dynamics is not unitary, we do \textit{not} expect that (whilst it is being measured) the quantum state should transform under a unitary representation of the Lorentz/Poincare group, but instead the time component should include the fact that the evolution is stochastic in Equation \eqref{eq: statefield}. An obvious example of this is the fact that when a measurement is being performed time-translations are generated by Equation \eqref{eq: statefield} which is non-unitary, nor is it linear. 
However, even though the dynamics is in general stochastic and non-unitary, the quantum state remains pure on any realization of the noise process and so purity is preserved. One drawback of the path integral approach is that though it tells us that the dynamics is Lorentz invariant, it does not tell us explicitly how to transform initial states between frames. The physical relevance of transforming quantum states between is a subtle point, since we only ever infer about the existence of quantum states by observing classical measurement outcomes and signals. Since we know how the measurement $z(x)$ transform - as Lorentz scalars - and we know the dynamics is Lorentz invariant, this should be sufficient to derive how the quantum states transform between frames, but it is not immediately obvious how to proceed mathematically. Note within this framework deriving how the quantum state transforms is really a consistency condition if we also ask that the measurement signal is an objective Lorentz scalar. To see this, consider two observers in Lorentz related frames who see a classical measurement field $z:M\to \mathbb{R}$ in there respective frames $z_A(x_A), z_B(x_B)$. They monitor there values to make inferences about the quantum state of the system. Eventually, by performing measurements and looking at the values of their fields, they will have each inferred that the quantum states $|\psi_A(z_A)\rangle, |\psi_B(z_B) \rangle$. Since $z_A$ and $z_B$ are related by a Lorentz transformation, and their evolution depends on $|\psi_A(z_A)\rangle, |\psi_B(z_B) \rangle$ this should (formally) be enough to determine how the quantum state transforms between frame. For example by solving the inverse problem for $|\psi_A(z_A)$, given knowledge of the $z_B$, the frame transformation to the boosted observer, and $|\psi_B(z_B) \rangle$. t would be interesting to flesh out the dynamics introduced in Equation \eqref{eq: LorentzInvariantActionMeasurement} further, and in particular to try and construct the generators generating the Lorentz transformations. 
